FoCTTA: Low-Memory Continual Test-Time Adaptation with Focus

Continual adaptation to domain shifts at test time (CTTA) is crucial for enhancing the intelligence of deep learning enabled IoT applications. However, prevailing TTA methods, which typically update all batch normalization (BN) layers, exhibit two memory inefficiencies. First, the reliance on BN layers for adaptation necessitates large batch sizes, leading to high memory usage. Second, updating all BN layers requires storing the activations of all BN layers for backpropagation, exacerbating the memory demand. Both factors lead to substantial memory costs, making existing solutions impractical for IoT devices. In this paper, we present FoCTTA, a low-memory CTTA strategy. The key is to automatically identify and adapt a few drift-sensitive representation layers, rather than blindly update all BN layers. The shift from BN to representation layers eliminates the need for large batch sizes. Also, by updating adaptation-critical layers only, FoCTTA avoids storing excessive activations. This focused adaptation approach ensures that FoCTTA is not only memory-efficient but also maintains effective adaptation. Evaluations show that FoCTTA improves the adaptation accuracy over the state-of-the-arts by 4.5%, 4.9%, and 14.8% on CIFAR10-C, CIFAR100-C, and ImageNet-C under the same memory constraints. Across various batch sizes, FoCTTA reduces the memory usage by 3-fold on average, while improving the accuracy by 8.1%, 3.6%, and 0.2%, respectively, on the three datasets.

==> checklist.tex <==
\section{AAAI Paper Checklist}


\begin{enumerate}

\item {\bf This paper:}
    \item[] Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes)
\item[] Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes)
\item[] Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes)


\item {\bf Does this paper make theoretical contributions? (No)}


\item {\bf Does this paper rely on one or more datasets? (yes)}

   \item[] A motivation is given for why the experiments are conducted on the selected datasets (yes)
\item[] All novel datasets introduced in this paper are included in a data appendix. (NA)
\item[] All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (NA)
\item[] All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes)
\item[] All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes)
\item[] All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (NA)

\item {\bf Does this paper include computational experiments? (yes)}

\item[]  Any code required for pre-processing data is included in the appendix. (no).
\item[]  All source code required for conducting and analyzing the experiments is included in a code appendix. (no)
\item[]  All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)
\item[]  All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes)
\item[]  If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes)
\item[]  This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes)
\item[] This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes)
\item[]  This paper states the number of algorithm runs used to compute each reported result. (yes)
\item[]  Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes)
\item[]  The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes)
\item[]  This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (NA)
\item[]  This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes)


\end{enumerate}


